Linearly Implicit Multistep Methods for Time Integration

Time integration methods for solving initial value problems are an important component of many scientific and engineering simulations. Implicit time integrators are desirable for their stability properties, significantly relaxing restrictions on timestep size. However, implicit methods require solutions to one or more systems of nonlinear equations at each timestep, which for large simulations can be prohibitively expensive. This paper introduces a new family of linearly implicit multistep methods (LIMM), which only requires the solution of one linear system per timestep. Order conditions and stability theory for these methods are presented, as well as design and implementation considerations. Practical methods of order up to five are developed that have similar error coefficients, but improved stability regions, when compared to the widely used BDF methods. Numerical testing of a self-starting variable stepsize and variable order implementation of the new LIMM methods shows measurable performance improvement over a similar BDF implementation.

==> Tables/LIMM_variable_coefficients_5.tex <==
\begin{array}{c|l}
\hline
 \alpha_{-1} & 1 \\
 \beta_{-1} & 0 \\
 \mu_{-1} & \left[3 \alpha_1 c_1^5-5 \alpha_1 \left(c_2+c_3\right) c_1^4+10 \alpha_1 c_2 c_3 c_1^3-5 c_1 \left(\alpha_2 c_2^4-2 \alpha_2 c_3 c_2^3-2 c_2 \left(\alpha_3 c_3^3-3 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right)+2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+2\right)+\alpha_3 c_3^4+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4 \right.\right. \\ & \left.\left. -4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)-3\right)+3 \alpha_2 c_2^5-5 \alpha_2 c_2^4 c_3-5 c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right) \right. \\ & \left. +3 \left(\alpha_3 c_3^5-5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+4\right)\right]/\left(60 \left(c_1+1\right) \left(c_2+1\right) \left(c_3+1\right)\right) \\
\hline
 \alpha_0 & -104367911/41202283 \\
 \beta_0 & 60/137 \\
 \mu_0 & \left[-3 \alpha_1 c_1^5+5 \left(c_2+c_3-1\right) \alpha_1 c_1^4-10 \left(c_2 \left(c_3-1\right)-c_3\right) \alpha_1 c_1^3-30 c_2 c_3 \alpha_1 c_1^2+5 \left(\alpha_2 c_2^4-2 \left(c_3-1\right) \alpha_2 c_2^3-6 c_3 \alpha_2 c_2^2-2 \left(\alpha_3 c_3^3+3 \alpha_3 c_3^2-3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4-2 \beta_0+1\right) c_3+2 c_4^3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+3 c_4^2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right) c_2+3 c_4^4+4 c_4^3+3 c_4^4 \alpha_0+4 c_4^3 \alpha_0+3 c_4^4 \alpha_1+4 c_4^3 \alpha_1+3 c_4^4 \alpha_2+4 c_4^3 \alpha_2+c_3^4 \alpha_3 \right.\right. \\ & \left.\left. +3 c_4^4 \alpha_3+2 c_3^3 \alpha_3+4 c_4^3 \alpha_3-2 c_3 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right)+1\right) c_1-12 c_4^5+15 c_3 c_4^4-15 c_4^4+20 c_3 c_4^3+5 c_3-12 c_4^5 \alpha_0+15 c_3 c_4^4 \alpha_0-15 c_4^4 \alpha_0+20 c_3 c_4^3 \alpha_0 \right. \\ & \left. -12 c_4^5 \alpha_1+15 c_3 c_4^4 \alpha_1-15 c_4^4 \alpha_1+20 c_3 c_4^3 \alpha_1-3 c_2^5 \alpha_2-12 c_4^5 \alpha_2+15 c_3 c_4^4 \alpha_2-15 c_4^4 \alpha_2+20 c_3 c_4^3 \alpha_2+5 c_2^4 \left(c_3-1\right) \alpha_2+10 c_2^3 c_3 \alpha_2-3 c_3^5 \alpha_3-12 c_4^5 \alpha_3-5 c_3^4 \alpha_3+15 c_3 c_4^4 \alpha_3-15 c_4^4 \alpha_3+20 c_3 c_4^3 \alpha_3 \right. \\ & \left.+5 c_2 \left(\alpha_3 c_3^4+2 \alpha_3 c_3^3-2 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4 c_4^3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+1\right)+3\right]/\left(60 c_1 c_2 c_3\right) \\
\hline
 \alpha_1 & 59680231/21017185 \\
 \beta_1 & \left[-5 c_2^2 \left(4 c_3^2 \left(\alpha_1 c_1^3-3 \alpha_1 c_4^2 c_1+2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right)+\alpha_3 c_3^5+\alpha_3 c_4 c_3^4-8 \alpha_3 c_4^2 c_3^3-c_3 \left(3 \alpha_1 c_1^4-4 \alpha_1 c_4 c_1^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right) \right.\right. \\ & \left.\left. -c_4 \left(3 \alpha_1 c_1^4-4 \alpha_1 c_4 c_1^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)\right)+3 \alpha_2 \left(c_3+c_4\right) c_2^6-\alpha_2 \left(5 c_3^2+2 c_4 c_3+5 c_4^2\right) c_2^5-5 \alpha_2 c_3 c_4 \left(c_3+c_4\right) c_2^4+40 \alpha_2 c_3^2 c_4^2 c_2^3+\left(c_3+c_4\right) c_2 \left(-12 \alpha_1 c_1^5 \right.\right. \\ & \left.\left. +15 \alpha_1 \left(c_3+c_4\right) c_1^4-20 \alpha_1 c_3 c_4 c_1^3+3 \alpha_3 c_3^5-5 \alpha_3 c_3^4 c_4-3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)+15 c_4+12\right)+c_3 c_4 \left(-12 \alpha_1 c_1^5+15 \alpha_1 \left(c_3+c_4\right) c_1^4 \right.\right. \\ & \left.\left. -20 \alpha_1 c_3 c_4 c_1^3+3 \alpha_3 c_3^5-5 \alpha_3 c_3^4 c_4-3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)+15 c_4+12\right)\right] \\ & /\left(60 \left(c_1-c_2\right) \left(c_1-c_3\right) \left(c_1-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
 \mu_1 & \left[-3 \left(c_3 c_4 \left(c_4+1\right)+c_2 \left(c_4^2+c_4+c_3\right)\right) \alpha_1 c_1^6+\left(5 \left(c_4^2+c_4+c_3\right) c_2^2+c_3 \left(5 c_3+2 c_4 \left(c_4+5\right)\right) c_2+5 c_3^2 c_4 \left(c_4+1\right)\right) \alpha_1 c_1^5-5 c_2 c_3 \left(c_4 \left(c_4-c_3 \left(c_4-2\right)\right)+c_2 \left(2 c_3-\left(c_4-2\right) c_4\right)\right) \alpha_1 c_1^4 \right. \\ & \left. +10 c_2 c_3 \left(c_2 \left(1-4 c_3\right)+c_3\right) c_4^2 \alpha_1 c_1^3+5 \left(\left(c_4^2+c_4+c_3\right) \alpha_2 c_2^5+c_3 \left(\left(c_4-1\right) c_4-2 c_3\right) \alpha_2 c_2^4-2 c_3^2 c_4 \left(4 c_4+1\right) \alpha_2 c_2^3-2 \left(\alpha_3 c_3^4+c_4 \left(4 c_4+1\right) \alpha_3 c_3^3-3 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +\left(\alpha_0+\alpha_2+\alpha_3-2 \beta_0+3\right) c_4^2-1\right) c_3^2-\left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right) c_3+2 c_4 \left(c_4+1\right) \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)\right) c_2^2+\left(\alpha_3 c_3^5+\left(c_4-1\right) c_4 \alpha_3 c_3^4 \right.\right.\right. \\ & \left.\left.\left. +2 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right) c_3^2-\left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4^2+8 c_4+3\right) c_3+3 c_4 \left(c_4+1\right) \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right)\right) c_2 \right.\right. \\ & \left.\left. +c_3 c_4 \left(c_4+1\right) \left(\alpha_3 c_3^4-4 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-3\right)\right) c_1^2-\left(3 \left(c_4^2+c_4+c_3\right) \alpha_2 c_2^6-c_3 \left(5 c_3+2 c_4 \left(c_4+1\right)\right) \alpha_2 c_2^5-5 c_3 c_4 \left(2 c_4+c_3 \left(c_4+1\right)\right) \alpha_2 c_2^4 \right.\right. \\ & \left.\left. +30 c_3^2 c_4^2 \alpha_2 c_2^3-5 \left(\alpha_3 c_3^5+c_4 \left(c_4+1\right) \alpha_3 c_3^4-6 c_4^2 \alpha_3 c_3^3+4 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right) c_3^2-\left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +3\right) c_3+3 c_4 \left(c_4+1\right) \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right)\right) c_2^2+\left(3 \alpha_3 c_3^6-2 c_4 \left(c_4+1\right) \alpha_3 c_3^5-10 c_4^2 \alpha_3 c_3^4+5 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4+3\right) c_3^2 \right.\right.\right. \\ & \left.\left.\left. -2 \left(15 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^6+19 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5-5 c_4^2-15 c_4-6\right) c_3+12 c_4 \left(c_4+1\right) \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+1\right)\right) c_2+3 c_3 c_4 \left(c_4+1\right) \left(\alpha_3 c_3^5 \right.\right.\right. \\ & \left.\left.\left. -5 \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right) c_3+4 c_4^5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4\right)\right) c_1+c_2 c_3 c_4^2 \left(-3 \alpha_2 c_2^5+5 \left(c_3-1\right) \alpha_2 c_2^4+10 c_3 \alpha_2 c_2^3+5 \left(\alpha_3 c_3^4+2 \alpha_3 c_3^3-2 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4 c_4^3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+1\right) c_2-3 c_3^5 \alpha_3-5 c_3^4 \alpha_3+5 c_3 \left(3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4 \right.\right.\right. \\ & \left.\left.\left. +4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)-3 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)\right)\right]/\left(60 c_1 \left(c_1+1\right) \left(c_1-c_2\right) \left(c_1-c_3\right) \left(c_1-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
\hline
 \alpha_2 & -97736124/57440479 \\
 \beta_2 & -\left[-5 c_1^2 \left(4 c_3^2 \left(\alpha_2 c_2^3-3 \alpha_2 c_4^2 c_2+2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right)+\alpha_3 c_3^5+\alpha_3 c_4 c_3^4-8 \alpha_3 c_4^2 c_3^3-c_3 \left(3 \alpha_2 c_2^4-4 \alpha_2 c_4 c_2^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right) \right.\right. \\ & \left.\left. -c_4 \left(3 \alpha_2 c_2^4-4 \alpha_2 c_4 c_2^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)\right)+3 \alpha_1 \left(c_3+c_4\right) c_1^6-\alpha_1 \left(5 c_3^2+2 c_4 c_3+5 c_4^2\right) c_1^5-5 \alpha_1 c_3 c_4 \left(c_3+c_4\right) c_1^4+40 \alpha_1 c_3^2 c_4^2 c_1^3+\left(c_3+c_4\right) c_1 \left(-12 \alpha_2 c_2^5 \right.\right. \\ & \left.\left. +15 \alpha_2 \left(c_3+c_4\right) c_2^4-20 \alpha_2 c_3 c_4 c_2^3+3 \alpha_3 c_3^5 -5 \alpha_3 c_3^4 c_4-3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)+15 c_4+12\right)+c_3 c_4 \left(-12 \alpha_2 c_2^5+15 \alpha_2 \left(c_3+c_4\right) c_2^4 \right.\right. \\ & \left.\left. -20 \alpha_2 c_3 c_4 c_2^3+3 \alpha_3 c_3^5-5 \alpha_3 c_3^4 c_4-3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)+15 c_4+12\right)\right] \\ & /\left(60 \left(c_1-c_2\right) \left(c_2-c_3\right) \left(c_2-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
 \mu_2 & \left[3 \left(c_3 c_4^2+c_2 \left(c_4^2+c_4+c_3\right)\right) \alpha_1 c_1^6-\left(5 \left(c_4^2+c_4+c_3\right) c_2^2+c_3 \left(5 c_3+2 c_4 \left(c_4+1\right)\right) c_2+5 \left(c_3-1\right) c_3 c_4^2\right) \alpha_1 c_1^5+5 c_3 \left(\left(-c_4^2+c_4+2 c_3\right) c_2^2-c_4 \left(2 c_4+c_3 \left(c_4+1\right)\right) c_2-2 c_3 c_4^2\right) \alpha_1 c_1^4 \right. \\ & \left. +10 c_2 c_3^2 c_4 \left(3 c_4+c_2 \left(4 c_4+1\right)\right) \alpha_1 c_1^3-5 \left(\left(c_4^2+c_4+c_3\right) \alpha_2 c_2^5+c_3 \left(\left(c_4-2\right) c_4-2 c_3\right) \alpha_2 c_2^4+2 \left(1-4 c_3\right) c_3 c_4^2 \alpha_2 c_2^3-2 \left(\alpha_3 c_3^4+c_4 \left(4 c_4+1\right) \alpha_3 c_3^3-3 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +\left(\alpha_0+\alpha_1+\alpha_3-2 \beta_0+3\right) c_4^2-1\right) c_3^2-\left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right) c_3+2 c_4 \left(c_4+1\right) \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)\right) c_2^2+\left(\alpha_3 c_3^5+c_4 \left(c_4+1\right) \alpha_3 c_3^4-6 c_4^2 \alpha_3 c_3^3 \right.\right.\right. \\ & \left.\left.\left. +4 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right) c_3^2-\left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4+3\right) c_3+3 c_4 \left(c_4+1\right) \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right)\right) c_2 \right.\right. \\ & \left.\left. +c_3 c_4^2 \left(\alpha_3 c_3^4+2 \alpha_3 c_3^3-2 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4 c_4^3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+1\right)\right) c_1^2+\left(3 \left(c_4^2+c_4+c_3\right) \alpha_2 c_2^6 \right.\right. \\ & \left.\left. -c_3 \left(5 c_3+2 c_4 \left(c_4+5\right)\right) \alpha_2 c_2^5+5 c_3 c_4 \left(c_4-c_3 \left(c_4-2\right)\right) \alpha_2 c_2^4-10 c_3^2 c_4^2 \alpha_2 c_2^3-5 \left(\alpha_3 c_3^5+\left(c_4-1\right) c_4 \alpha_3 c_3^4+2 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right) c_3^2-\left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4^2+8 c_4+3\right) c_3+3 c_4 \left(c_4+1\right) \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right)\right) c_2^2+\left(3 \alpha_3 c_3^6-2 c_4 \left(c_4+1\right) \alpha_3 c_3^5-10 c_4^2 \alpha_3 c_3^4+5 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4+3\right) c_3^2-2 \left(15 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^6+19 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5-5 c_4^2-15 c_4-6\right) c_3+12 c_4 \left(c_4+1\right) \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+1\right)\right) c_2 \right.\right. \\ & \left.\left. +c_3 c_4^2 \left(3 \alpha_3 c_3^5+5 \alpha_3 c_3^4-5 \left(3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) c_3+3 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)\right)\right) c_1 \right. \\ & \left. +c_2 c_3 c_4 \left(c_4+1\right) \left(3 \alpha_2 c_2^5-5 c_3 \alpha_2 c_2^4-5 \left(\alpha_3 c_3^4-4 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-3\right) c_2+3 \left(\alpha_3 c_3^5-5 \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right) c_3 \right.\right.\right. \\ & \left.\left.\left. +4 c_4^5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4\right)\right)\right]/\left(60 \left(c_1-c_2\right) c_2 \left(c_2+1\right) \left(c_2-c_3\right) \left(c_2-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
\hline
 \alpha_3 & 19515650/39801941 \\
 \beta_3 & -\left[-5 c_1^2 \left(4 c_2^2 \left(\alpha_3 c_3^3-3 \alpha_3 c_4^2 c_3+2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right)+\alpha_2 c_2^5+\alpha_2 c_4 c_2^4-8 \alpha_2 c_4^2 c_2^3-c_2 \left(3 \alpha_3 c_3^4-4 \alpha_3 c_4 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right) \right.\right. \\ & \left.\left. -c_4 \left(3 \alpha_3 c_3^4-4 \alpha_3 c_4 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)\right)+3 \alpha_1 \left(c_2+c_4\right) c_1^6-\alpha_1 \left(5 c_2^2+2 c_4 c_2+5 c_4^2\right) c_1^5-5 \alpha_1 c_2 c_4 \left(c_2+c_4\right) c_1^4+40 \alpha_1 c_2^2 c_4^2 c_1^3 \right. \\ & \left. +\left(c_2+c_4\right) c_1 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_4 c_2^4+5 c_2 \left(3 \alpha_3 c_3^4-4 \alpha_3 c_4 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)-3 \left(4 \alpha_3 c_3^5-5 \alpha_3 c_4 c_3^4+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5-5 c_4-4\right)\right) \right. \\ & \left. +c_2 c_4 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_4 c_2^4+5 c_2 \left(3 \alpha_3 c_3^4-4 \alpha_3 c_4 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4+3\right)-3 \left(4 \alpha_3 c_3^5-5 \alpha_3 c_4 c_3^4+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5-5 c_4-4\right)\right)\right] \\ & /\left(60 \left(c_1-c_3\right) \left(c_3-c_2\right) \left(c_3-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
 \mu_3 & \left[3 \left(c_3 c_4 \left(c_4+1\right)+c_2 \left(c_4^2+c_3\right)\right) \alpha_1 c_1^6-\left(5 \left(c_4^2+c_3\right) c_2^2+\left(5 c_3^2+2 c_4 \left(c_4+1\right) c_3-5 c_4^2\right) c_2+5 c_3^2 c_4 \left(c_4+1\right)\right) \alpha_1 c_1^5+5 c_2 \left(c_3 \left(-c_3 \left(c_4-1\right)-2 c_4\right) c_4+c_2 \left(2 c_3^2-c_4 \left(c_4+1\right) c_3-2 c_4^2\right)\right) \alpha_1 c_1^4 \right. \\ & \left. +10 c_2^2 c_3 c_4 \left(3 c_4+c_3 \left(4 c_4+1\right)\right) \alpha_1 c_1^3-5 \left(\left(c_4^2+c_3\right) \alpha_2 c_2^5+\left(-2 c_3^2+c_4 \left(c_4+1\right) c_3+2 c_4^2\right) \alpha_2 c_2^4-2 c_3 c_4 \left(3 c_4+c_3 \left(4 c_4+1\right)\right) \alpha_2 c_2^3-2 \left(\alpha_3 c_3^4+4 c_4^2 \alpha_3 c_3^3-3 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +\left(\alpha_0+\alpha_1+\alpha_2-2 \beta_0+3\right) c_4^2-1\right) c_3^2-2 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 \left(\beta_0-1\right) c_4^2-1\right) c_3+c_4^2 \left(2 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^2-1\right)\right) c_2^2 \right.\right. \\ & \left.\left. +\left(3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^6+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+2 c_3^3 \alpha_3 c_4^2+c_4^2+c_3^4 \left(c_4-2\right) \alpha_3 c_4+c_3^5 \alpha_3+2 c_3^2 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right)-c_3 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5 \right.\right.\right.\right. \\ & \left.\left.\left.\left. +7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4+3\right)\right) c_2+c_3 c_4 \left(c_4+1\right) \left(\alpha_3 c_3^4-4 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-3\right)\right) c_1^2+\left(3 \left(c_4^2+c_3\right) \alpha_2 c_2^6 \right.\right. \\ & \left.\left. -\left(5 c_3^2+2 c_4 \left(c_4+1\right) c_3-5 c_4^2\right) \alpha_2 c_2^5-5 c_3 c_4 \left(c_3 \left(c_4-1\right)+2 c_4\right) \alpha_2 c_2^4-5 \left(3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^6+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+2 c_3^3 \alpha_3 c_4^2+c_4^2+c_3^4 \left(c_4-2\right) \alpha_3 c_4+c_3^5 \alpha_3 \right.\right.\right. \\ & \left.\left.\left. +2 c_3^2 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3-3 c_4-2\right)-c_3 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+7 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-2 c_4^2+4 c_4+3\right)\right) c_2^2+\left(3 \alpha_3 c_3^6-2 c_4 \left(c_4+5\right) \alpha_3 c_3^5+5 c_4^2 \alpha_3 c_3^4 \right.\right.\right. \\ & \left.\left.\left. +5 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4+4 c_4^2+8 c_4+3\right) c_3^2-2 \left(15 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^6+19 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5-5 c_4^2-15 c_4-6\right) c_3 \right.\right.\right. \\ & \left.\left.\left. +3 c_4^2 \left(4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)\right) c_2+3 c_3 c_4 \left(c_4+1\right) \left(\alpha_3 c_3^5-5 \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right) c_3+4 c_4^5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4\right)\right) c_1 \right. \\ & \left. +c_2 c_3 c_4 \left(c_4+1\right) \left(3 \alpha_2 c_2^5-5 c_3 \alpha_2 c_2^4-5 \left(\alpha_3 c_3^4-4 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) c_3+3 c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-3\right) c_2+3 \left(\alpha_3 c_3^5-5 \left(c_4^4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)-1\right) c_3 \right.\right.\right. \\ & \left.\left.\left. +4 c_4^5 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right)+4\right)\right)\right]/\left(60 \left(c_1-c_3\right) c_3 \left(c_3+1\right) \left(c_3-c_2\right) \left(c_3-c_4\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
\hline
 \alpha_4 & -188732392210474496577705869057/1979785468648998861857945444345 \\
 \beta_4 & -\left[-5 c_1^2 \left(-4 c_2^2 \left(3 c_3^2 \left(\beta_0+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) \left(-c_4\right)-1\right)+2 \alpha_3 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+\alpha_2 c_2^5+\alpha_2 c_3 c_2^4-8 \alpha_2 c_3^2 c_2^3+c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) \right.\right.\right. \\ & \left.\left.\left. +3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)+c_3 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)\right)+3 \alpha_1 \left(c_2+c_3\right) c_1^6-\alpha_1 \left(5 c_2^2+2 c_3 c_2+5 c_3^2\right) c_1^5 \right. \\ & \left. -5 \alpha_1 c_2 c_3 \left(c_2+c_3\right) c_1^4+40 \alpha_1 c_2^2 c_3^2 c_1^3+\left(c_2+c_3\right) c_1 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_3 c_2^4-5 c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right) \right.\right. \\ & \left.\left. +3 \left(\alpha_3 c_3^5-5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+4\right)\right)+c_2 c_3 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_3 c_2^4-5 c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) \right.\right.\right. \\ & \left.\left.\left. +3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)+3 \left(\alpha_3 c_3^5-5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+4\right)\right)\right] \\ & /\left(60 \left(c_2-c_4\right) \left(c_4-c_1\right) \left(c_4-c_3\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
 \mu_4 & \left[-5 c_1^2 \left(-4 c_2^2 \left(3 c_3^2 \left(\beta_0+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) \left(-c_4\right)-1\right)+2 \alpha_3 c_3^3+\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+\alpha_2 c_2^5+\alpha_2 c_3 c_2^4-8 \alpha_2 c_3^2 c_2^3+c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) \right.\right.\right. \\ & \left.\left.\left. +3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)+c_3 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)\right)+3 \alpha_1 \left(c_2+c_3\right) c_1^6-\alpha_1 \left(5 c_2^2+2 c_3 c_2+5 c_3^2\right) c_1^5 \right. \\ & \left. -5 \alpha_1 c_2 c_3 \left(c_2+c_3\right) c_1^4+40 \alpha_1 c_2^2 c_3^2 c_1^3+\left(c_2+c_3\right) c_1 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_3 c_2^4-5 c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right)+3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right) \right.\right. \\ & \left.\left. +3 \left(\alpha_3 c_3^5-5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+4\right)\right)+c_2 c_3 \left(3 \alpha_2 c_2^5-5 \alpha_2 c_3 c_2^4-5 c_2 \left(\alpha_3 c_3^4-4 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^3+1\right) \right.\right.\right. \\ & \left.\left.\left. +3 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-3\right)+3 \left(\alpha_3 c_3^5-5 c_3 \left(\left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^4-1\right)+4 \left(\alpha_0+\alpha_1+\alpha_2+\alpha_3+1\right) c_4^5+4\right)\right)\right] \\ & /\left(60 \left(c_2-c_4\right) \left(c_4-c_1\right) \left(c_4-c_3\right) \left(c_2 c_3 c_4+c_1 \left(c_3 c_4+c_2 \left(c_3+c_4\right)\right)\right)\right) \\
\end{array}

